Towards Realistic Single-Task Continuous Learning Research for NER

There is an increasing interest in continuous learning (CL), as data privacy is becoming a priority for real-world machine learning applications. Meanwhile, there is still a lack of academic NLP benchmarks that are applicable for realistic CL settings, which is a major challenge for the advancement of the field. In this paper we discuss some of the unrealistic data characteristics of public datasets, study the challenges of realistic single-task continuous learning as well as the effectiveness of data rehearsal as a way to mitigate accuracy loss. We construct a CL NER dataset from an existing publicly available dataset and release it along with the code to the research community.

==> figures/skewed_results_train_test.tex <==
\begin{figure*}[]
    \begin{floatrow}
    \capbtabbox{%

        \begin{tabular}{*{4}{c}}
        \toprule
        & \small Overall & \small CodeBlock & \small DataStruct. \\
        \midrule
        \small Baseline (non-CL) & 51.76 & 13.89  & 45.98 \\
        \small CL w/o Replay & 44.95 & 0.00 & 34.28 \\
        \small CL w/ Replay  & 48.94 & 9.42 & 33.93 \\
        \bottomrule
        \end{tabular}
        \vspace{3em}
        
    \label{tab:so-all-results}
    }{%
        \caption{Overall and selected entity type F1 scores after training incrementally over all 5 skewed episodes vs on all training data at once. Scores are averaged over all 5 episodes' test sets.}    
    }
    \ffigbox{%
        \includegraphics[width=0.45\textwidth]{images/skewed_tests_on_train_over_time.png}
        \label{fig:forget-on-train}
    }{%
        \caption{Overall F1 score evaluated on each of the 5 Train episodes. All models are trained on data from all episodes. The CL models are trained incrementally, starting with episode 1 and finishing with episode 5.}
    }
    \end{floatrow}
\end{figure*}

==> figures/so-forget-on-test-temp.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/Temporal_tests_over_time.png}
    \caption{Overall F1 score evaluated on each of the 5 Test episodes from the temporal split. All models evaluated here are trained on data from all episodes, where the CL models are trained incrementally, starting with episode 1 and finishing with episode 5.}
    \label{fig:forget-on-test-temp}
\end{figure}

==> figures/so-forget-on-test.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/Skewed_tests_over_time.png}
    \caption{Overall F1 score evaluated on each of the 5 Test episodes from the skewed split. All models evaluated here are trained on data from all episodes, where the CL models are trained incrementally, starting with episode 1 and finishing with episode 5.}
    \label{fig:forget-on-test}
\end{figure}


==> figures/so-forget-on-train-temp.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/Temporal_tests_on_train_over_time.png}
    \caption{Overall F1 score evaluated on each of the 5 Train episodes from the temporal split. All models evaluated here are trained on data from all episodes, where the CL models are trained incrementally, starting with episode 1 and finishing with episode 5.}
    \label{fig:forget-on-train-temp}
\end{figure}

==> figures/so-forget-on-train.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/Skewed_tests_on_train_over_time.png}
    \caption{Overall F1 score evaluated on each of the 5 Train episodes from the skewed split. All models evaluated here are trained on data from all episodes, where the CL models are trained incrementally, starting with episode 1 and finishing with episode 5.}
    \label{fig:forget-on-train}
\end{figure}

==> figures/so-orig-dist.tex <==
\begin{figure*}[!tp]
    \centering
    \includegraphics[width=1.0\textwidth]{images/so-orig-train-dist-no-counts.pdf}
    \caption{Entity type distribution across episodes in the original Stackoverflow dataset after splitting it to time-based episodes.  Each vertical bar has the frequency for each of the 5 episodes. For readability we removed a few types with low counts in all episodes.}
    \label{fig:mst_sitelinks}
\end{figure*}

==> figures/so-skewed-dist.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.0\textwidth]{images/so-skewed-train-dist.pdf}
    \caption{Entity type distribution across episodes in the skewed Stackoverflow dataset that we propose.  Each vertical bar has the frequency for each of the 5 episodes. For readability we removed types with low counts in each episode.}
    \label{fig:mst_sitelinks}
\end{figure*}

==> tables/episode_stats.tex <==
\begin{table*}[!tp]
    \centering
        \begin{tabular}{*{7}{c}}
        \toprule
       
        & \small Ep. 1 & \small Ep. 2 & \small Ep. 3 & \small Ep. 4 & \small Ep. 5 & \small Total \\
        \midrule
        Time-Based, Train & 2551 & 2444 & 2243 & 2450 & 2386 & 12074 \\
Distribution-Based, Train & 2267 & 2358 & 3134 & 2231 & 1499 & 11489 \\
\midrule
Time-Based, Test & 775 & 665 & 521 & 496 & 632 & 3089 \\
Distribution-Based, Test & 532 & 600 & 493 & 792 & 514 & 2931 \\
        \bottomrule
        \end{tabular}
        \caption{Episode Sizes for Time-Based and Distribution-Based Episodes}
    \label{tab:episode_stats}
    \end{table*}



==> tables/replay_hurts.tex <==
\begin{table*}[!tp]
    \centering
        \begin{tabularx}{\textwidth}{c|c}
        \toprule
       Example & Replay \\
       \midrule
        \makecell{...transfer file XXX with size YYYY... \\ \hspace{2.0em} File\_Name \hspace{3.0em} Value \\ \hspace{4.0em} Value \hspace{5.0em} Value} & \makecell{...yum update XXX will cause the process crash... \\ Application Value} \\
        \midrule
        \makecell{...link those C files... \\ Language \\ \hspace{4.0em} File\_Type} & \makecell{...each mat file is different... \\ File\_Type} \\
        \midrule
        \makecell{...have the config set to only run 1 server instead... \\ \hspace{2.0em} Device \\ \hspace{4.0em} Application \hspace{5.0em} Value} & \makecell{...doesn't require a particular server-side infrastructure... \\ Device} \\
        % 1& 8/4/2008 -- 6/26/2012 & 2333 / 235 \\
        %  2& 6/27/2012 -- 3/13/2014 & \\
        %   3& 3/14/2014 -- 6/27/2015 & \\
        %    4& 6/28/2015 -- 10/1/2016 & \\
        %     5& 10/2/2016 -- 3/27/2018 & \\
        %\midrule

        \bottomrule
        \end{tabularx}
        \caption{Training examples which were incorrectly predicted (after training on all 5 episodes) by the continual learning model with replay, but correctly predicted by CL without replay. All examples are taken from episode 1 of the time-based episode setting. The first example shows an uncommon token which is memorized incorrectly based on one instance in the replayed data. The second example shows a construction which is memorized and applied incorrectly from the replayed data. The third example shows a replayed example that is not representative of the training data - ``server'' is typically an Application.}
    \label{tab:replay_hurts}
    \end{table*}


==> tables/replay_still_fails.tex <==
\begin{table*}[!tp]
    \centering
        \begin{tabularx}{\textwidth}{p{0.33\textwidth}|p{0.33\textwidth}|p{0.33\textwidth}}
        \toprule
       Correct & Predicted & Explanation \\
       \midrule
       How to set an id to [\textbf{Library\_Class} EditText(Android)] when working with [\textbf{Library} Cordova]? & How to set an [\textbf{Variable\_Name} id] to [\textbf{Library\_Class} EditText(Android)] when working with [\textbf{Library} Cordova]? & The example ``I removed the [\textbf{Code\_Block} \%d] from the [\textbf{Variable\_Name} id] section of your code'' is replayed, leading to incorrect memorization. \\
       \midrule
       I have created screenshots of the [\textbf{Application} Layout Editor] of [\textbf{Application} Android Studio] & I have created screenshots of the [\textbf{Application} Layout Editor] of [\textbf{Operating\_System} Andriod] [\textbf{Application} Studio] & Android as an \textbf{Operating\_System} is very common in episode 5, but the \textbf{Application} Andriod Studio is not included in replay from episode 1. \textbf{Application} is much more common in episode 1 than episode 5 overall. \\

       \midrule
       As this needs to be done for each [\textbf{Data\_Type} date], it can be done using [\textbf{Code\_Block} cursor]. & As this needs to be done for each date, it can be done using [\textbf{Library\_Function} cursor]. & ``Date'' is never used as a \textbf{Data\_Type} in episode 5. Also, \textbf{Code\_Block} is generally uncommon in episode 5 but very common in episode 1. \\
        % \makecell{...transfer file XXX with size YYYY... \\ \hspace{2.0em} File\_Name \hspace{3.0em} Value \\ \hspace{4.0em} Value \hspace{5.0em} Value} & \makecell{...yum update XXX will cause the process crash... \\ Application Value} \\
        % \midrule
        % \makecell{...link those C files... \\ Language \\ \hspace{4.0em} File\_Type} & \makecell{...each mat file is different... \\ File\_Type} \\
        % \midrule
        % \makecell{...have the config set to only run 1 server instead... \\ \hspace{2.0em} Device \\ \hspace{4.0em} Application \hspace{5.0em} Value} & \makecell{...doesn't require a particular server-side infrastructure... \\ Device} \\
        % 1& 8/4/2008 -- 6/26/2012 & 2333 / 235 \\
        %  2& 6/27/2012 -- 3/13/2014 & \\
        %   3& 3/14/2014 -- 6/27/2015 & \\
        %    4& 6/28/2015 -- 10/1/2016 & \\
        %     5& 10/2/2016 -- 3/27/2018 & \\
        %\midrule

        \bottomrule
        \end{tabularx}
        \caption{Training examples which were incorrectly predicted (after training on all 5 episodes) by the continual learning model with replay, but correctly predicted by the baseline model. All examples are taken from episode 1 of the non-stationary episode setting. }
    \label{tab:replay_still_fails}
    \end{table*}


==> tables/so-orig-overall-results.tex <==
\begin{table}[!tp]
    \centering
        \begin{tabular}{*{5}{c}}
        \toprule
        & & \small Overall & \small CodeBlock & \small DataStruct.  \\
        \midrule
        & Baseline (non-CL) & 51.36 & 25.67 & 75.27 \\
        Temporal & CL w/o Replay & 51.52 & 28.59 & 73.76 \\
        & CL w/ Real Replay & 51.12 & 26.41 & 72.82 \\
        \bottomrule
        \end{tabular}
        \caption{Overall F1 scores after training incrementally over all 5 temporal episodes vs on all training data at once. Scores are averaged over all 5 episodes' test sets.}
    \label{tab:results-temporal}
    \end{table}



